Implementation and Synthesis of Math Library Functions

Achieving speed and accuracy for math library functions like exp, sin, and log is difficult. This is because low-level implementation languages like C do not help math library developers catch mathematical errors, build implementations incrementally, or separate high-level and low-level decision making. This ultimately puts development of such functions out of reach for all but the most experienced experts. To address this, we introduce MegaLibm, a domain-specific language for implementing, testing, and tuning math library implementations. MegaLibm is safe, modular, and tunable. Implementations in MegaLibm can automatically detect mathematical mistakes like sign flips via semantic wellformedness checks, and components like range reductions can be implemented in a modular, composable way, simplifying implementations. Once the high-level algorithm is done, tuning parameters like working precisions and evaluation schemes can be adjusted through orthogonal tuning parameters to achieve the desired speed and accuracy. MegaLibm also enables math library developers to work interactively, compiling, testing, and tuning their implementations and invoking tools like Sollya and type-directed synthesis to complete components and synthesize entire implementations. MegaLibm can express 8 state-of-the-art math library implementations with comparable speed and accuracy to the original C code, and can synthesize 5 variations and 3 from-scratch implementations with minimal guidance.

==> latexpand <==
#!/usr/bin/perl
# Inspired by latexpand by D. Musliner, University of Michigan
# 2012, 2013, 2014, 2015, 2016, 2017: Matthieu Moy <git@matthieu-moy.fr>
# BSD License

use strict;
use Cwd;
use Getopt::Long;
use IO::Handle;
use File::Spec;

my $TEXINPUTS = $ENV{'TEXINPUTS'};
if (!$TEXINPUTS) { $TEXINPUTS = getcwd(); }

my $verbose;
my $keep_comments;
my $keep_includes;
my $empty_comments;
my $help;
my $long_help;
my $output;
my $explain;
my $show_graphics;
my $graphics_extensions = ":.pdf:.png:.jpg:.eps";
my $expand_usepackage;
my $expand_bbl;
my $fatal;
my $version;
my $makeatletter;
my $inside_import;

GetOptions (
    'h' => \$help,
    'help' => \$long_help,
    'verbose|v' => \$verbose,
    'keep-comments' => \$keep_comments,
    'keep-includes' => \$keep_includes,
    'empty-comments' => \$empty_comments,
    'output|o=s' => \$output,
    'explain' => \$explain,
    'show-graphics' => \$show_graphics,
    'graphics-extensions' => \$graphics_extensions,
    'expand-usepackage' => \$expand_usepackage,
    'expand-bbl=s' => \$expand_bbl,
    'fatal' => \$fatal,
    'version' => \$version,
        'makeatletter' => \$makeatletter,
) or pod2usage_wrapper(2);
version() if $version;
pod2usage_wrapper(0) if $help;
pod2usage_wrapper(-exitstatus => 0, -output => \*STDOUT, -verbose => 2) if $long_help;

sub pod2usage_wrapper
{
    # Like pod2usage, but fall back to a simpler implem in case
    # pod2usage can't be found.
    if  (eval {require Pod::Usage;1;} ne 1) {
        print "Please install perldoc and Pod::Usage to get proper help.\n";
        my $started = 0;
        open (my $in, '<', "$0") or die $!;
        while (<$in>) {
            if ($started) {
                print;
            }
            if (/^__END__$/) {
                $started = 1;
            }
        }
    } else {
        Pod::Usage->import();
        pod2usage(@_);
    }
}

sub get_version
{
    # $VERSION's value will be substituted by 'make dist', but the
    # next line won't (the string has to be broken to avoid it).
    my $VERSION = 'v1.4-1-gb32a776';
    if ($VERSION eq '@LATEXPAND' . '_VERSION@') {
        my($vol,$dir,$file) = File::Spec->splitpath($0);
        chdir($dir);
        $VERSION = `git describe --tags HEAD 2>/dev/null`;
    }
    if ($VERSION eq '') {
        $VERSION = '<unknown version>';
    }
    $VERSION =~ s/^\s+|\s+$//g;
    return $VERSION;
}

sub version
{
    print "latexpand version ". get_version() .".\n";
    exit(0);
}

my $nl = "";
if ($empty_comments) {
    $nl = "%\n";
}

if ($output && $output ne "-") {
    open (my $OUTPUT, '>', "$output") or die $!;
    STDOUT->fdopen(\*$OUTPUT, 'w') or die $!;
}

sub say
{
    if ($verbose) {
        print STDERR "$_[0]";
    }
}

my $makeatletter_found;
my $in_preamble;

foreach my $file (@ARGV)
{
    say "processing $file\n";
    $makeatletter_found = 0;
    $in_preamble = 1;
        $inside_import = "";
    process_file($file, "  ");
}

sub process_file
{
    my $file = shift;
    my $prefix = (shift || "");
    my $in_comment = 0;
    open(my $FILE, "<", $file) or die "could not open input file '$file'\n";
    my $commented_newline = 0;
    while (my $line = <$FILE>) {
        if ($line =~ /^[ \t]*\\endinput/) {
            $line =~ s/(\\endinput.*)\n/% $1/;
            $in_comment = 1;
            process_line($line, $prefix, \$commented_newline);
            last;
        }
        process_line($line, $prefix, \$commented_newline, $file);
        if ($line =~ /^%.*[^\n]\z/ || $line =~ /[^\\]%.*[^\n]\z/) {
            # file ends with a comment not ending with a newline
            print "\n";
        }
        # Garbage at end of line after \end{document} is
        # ignored by LaTeX, but we don't allow anything before
        # to avoid e.g. \verb|\end{document}| from terminating
        # the file.
        if (!$keep_comments && $line =~ /^[ \t]*\\end\{document\}/) {
            last;
        }
    }
    close($FILE);
    return $in_comment;
}

sub process_line
{
    my ($line, $prefix, $commented_newline, $file) = @_;
    $_ = $line;
    if ($$commented_newline && /^\s*$/) {
        # Deal with:
        #
        # Line 1 % comment
        #
        # Line 2
        #
        # The newline after Line 1 is commented, but we still
        # want a new paragraph. We strip the comment together
        # with its newline, but re-add a newline to chnge
        # paragraph here if needed:
        print "\n";
    }
    $$commented_newline = 0;
    # Consider \makeatletter only in preamble, because we do want
    # to warn on \someCommand{\makeatletter\command@with@arobase}.
    if ($in_preamble && /^[^%]*\\makeatletter/) {
        $makeatletter_found = 1;
    }
    if ($in_preamble && /^[^%]*\\makeatother/) {
        $makeatletter_found = 0;
    }
    if (!$makeatletter && !$makeatletter_found
        && (my ($command) = /^[^%]*(\\[[:alpha:]]*@[[:alpha:]]*)/)) {
        print STDERR "Warning: command $command containing @ found in\n";
        print STDERR "Warning: $file.\n";
        print STDERR "Warning: consider using --makeatletter if the result is not compilable.\n";
    }
    unless ($keep_comments) {
        if (!$empty_comments) {
            # Include \n in pattern to avoid matching
            # comments at end of files

            # remove comments + whitespace-only lines completely
            if (s/^\s*%.*\n//) {
                $$commented_newline = 1;
            }

            # remove only the comment if the line has actual content
            if (s/([^\\])%.*\n/$1/) {
                $$commented_newline = 1;
            }
        }
        # Apply the "empty comments" treatment unconditionally
        # for end-of-files comments not matched above (it
        # doesn't harm to keep an empty comment sometimes, but
        # it may harm to leave a real comment if the goal was
        # to strip them).
        s/^%.*$/%/;
        s/([^\\])%.*$/$1%/;
    }

    unless ($keep_includes) {
        if (my ($before, $ignored, $full_filename, $after)
            = /^(([^%]|[^\\]%)*)\\include[{\s]+(.*?)[\s}](.*)$/) {
            $full_filename = find_tex_file($full_filename . ".tex");
            if ($full_filename) {
                say $prefix . "Found include for file: $full_filename\n";
                print $before . $nl;
                print '\clearpage{}' . $nl;
                print "% start include $full_filename\n" if ($explain);
                my $in_comment = process_file($full_filename, $prefix . "  ");
                if ($explain) {
                    print " % end include $full_filename\n";
                } elsif ($in_comment) {
                    print "\n";
                }
                print '\clearpage{}' . $nl;
                print $nl . $after . "\n";
                $_ = "";
            }
        } elsif (my ($before, $ignored, $full_filename, $after)
             = /^(([^%]|[^\\]%)*)\\input[{\s]+(.*?)[\s}](.*)$/) {
                        if ($inside_import) {
                              $full_filename = $inside_import . $full_filename;
                        }
            $full_filename = find_tex_file($full_filename, ":.tex");
            if ($full_filename) {
                say $prefix . "Found input for file: $full_filename\n";
                print $before . $nl;
                print "% start input $full_filename\n" if ($explain);
                my $in_comment = process_file($full_filename, $prefix . "  ");
                if ($explain) {
                    print " % end input $full_filename\n";
                } elsif ($in_comment) {
                    print "\n";
                }
                if ($after =~ /[^\s]/) {
                    # LaTeX produces this space, so let's do it also
                    print " " . $nl . $after . "\n";
                } else {
                    print " ";
                }
                $_ = "";
            }
        } elsif (my ($before, $ignored, $dir, $full_filename, $after)
             = /^(([^%]|[^\\]%)*)\\(?:sub)?import[{\s]+(.*?)[\s}][{\s]+(.*?)[\s}](.*)$/) {
                        if ($explain) {
                              print "% dir " . $dir ."\n";
                              print "% full_filename " . $full_filename ."\n";
                              print "% after " . $after ."\n";
                              print "% inside_import $inside_import\n";
                        }
                        $full_filename = $dir . $full_filename;
                        if ($inside_import) {
                              $full_filename = $inside_import . $full_filename;
                        }
                        print "% cat(inside_import,dir,full_filename) " . $full_filename ."\n" if ($explain);
            $full_filename = find_tex_file($full_filename, ":.tex");
            if ($full_filename) {
                say $prefix . "Found input for file: $full_filename\n";
                print $before . $nl;
                print "% start input $full_filename\n" if ($explain);
                                my $previous_import_dir = $inside_import;
                                $inside_import = $inside_import . $dir;
                my $in_comment = process_file($full_filename, $prefix . "  ");
                                $inside_import = $previous_import_dir;
                if ($explain) {
                    print " % end input $full_filename\n";
                } elsif ($in_comment) {
                    print "\n";
                }
                if ($after =~ /[^\s]/) {
                    # LaTeX produces this space, so let's do it also
                    print " " . $nl . $after . "\n";
                } else {
                    print " ";
                }
                $_ = "";
            }
        } elsif (my ($before, $ignored, $args, $full_filename, $after)
             = /^(([^%]|[^\\]%)*)\\includegraphics[\[\s]+(.*?)[\s\]][{\s]+(.*?)[\s}](.*)$/) {
                        if ($explain) {
                                print "% inside_import " . $inside_import ."\n";
                                print "% before " . $before ."\n";
                                print "% ignored " . $ignored ."\n";
                                print "% args " . $args ."\n";
                                print "% full_filename " . $full_filename ."\n";
                                print "% after " . $after ."\n";
                        }
                        if ($inside_import) {
                                $full_filename = $inside_import . $full_filename;
                                print "$before\\includegraphics[$args]{$full_filename}$after\n";
                                $_ = "";
                        }
        } elsif (my ($before, $ignored, $args, $full_filename, $after)
             = /^(([^%]|[^\\]%)*)\\lstinputlisting[\[\s]+(.*?)[\s\]][{\s]+(.*?)[\s}](.*)$/) {
                        if ($explain) {
                                print "% inside_import " . $inside_import ."\n";
                                print "% before " . $before ."\n";
                                print "% ignored " . $ignored ."\n";
                                print "% args " . $args ."\n";
                                print "% full_filename " . $full_filename ."\n";
                                print "% after " . $after ."\n";
                        }
                        if ($inside_import) {
                                $full_filename = $inside_import . $full_filename;
                                print "$before\\lstinputlisting[$args]{$full_filename}$after\n";
                                $_ = "";
                        }
        }
    }
    if ($expand_usepackage) {
        # Don't bother with before and after text, we just require the
        # usepackage to be alone on its line.
        if (my ($package_name) = /^\s*\\usepackage\{([^\}]*)\}\s*(%.*)?$/) {
            my $full = find_file($package_name . ".sty", $TEXINPUTS);
            if ($full) {
                say $prefix . "Found package file: $full\n";
                process_file($full, $prefix . "  ");
                $_ = "";
                # Forget about any commented newline
                # before the \usepackage:
                $$commented_newline = 0;
            } else {
                say $prefix . "Not including external package $package_name\n";
            }
        }
    }
    if ($expand_bbl) {
        if (my ($before, $bib_name, $after)
             = /^(.*)\\(?:bibliography|bibselect)\{([^\}]*)\}(.*)$/) {
            # The BBL file is not necessarily $bib_name.
            # Take it from the command-line.
            print $before . $nl;
            say $prefix . "Expanding BBL file: $expand_bbl\n";
            process_file($expand_bbl, $prefix . "  ");
            print " " . $nl . $after . "\n";
            $_ = "";
        }
    }
    if ($show_graphics) {
        if (/\\includegraphics(\[[^\]]*\])?{([^}]*)}/) {
                        my $full_filename = $2;
                        if ($inside_import) {
                                $full_filename = $inside_import . $full_filename;
                        }
            my $full = find_tex_file($full_filename, $graphics_extensions);
            say $prefix . "needs graphics file: ";
            print STDERR "$full\n";
        }
    }
    if (/^[ \t]*\\begin\{document\}/) {
        $in_preamble = 0;
        if ($makeatletter) {
            print '\makeatletter' . $nl;
        }
    }
    print;
}
# search $1 in $TEXINPUTS, with possible extensions in $2
sub find_tex_file
{
    my $file = shift;
    my $extensions = (shift || ":");
    foreach my $ext (split(':', $extensions, -1)) {
        my $full = find_file_global($file . $ext);
        if ($full) {
            return $full;
        }
    }
    if ($fatal) {
        die "ERROR: Could not find file [$file]\n";
    } else {
        print STDERR "Warning: Could not find file [$file]\n";
        return;
    }
}
sub find_file_global
{
    my $file = shift;
    if (open(my $fh, "-|", "kpsewhich", $file)) {
        my $full = <$fh>;
        chomp($full);
        close($fh);
        if ($full) {
            return $full;
        }
    }
    return find_file($file, $TEXINPUTS);
}
sub find_file
{
    my ($file, $path) = @_;
    if (File::Spec->file_name_is_absolute($file)) {
        if (-e "$file" && ! -d "$file") {
            return $file;
        } else {
            return;
        }
    }
    foreach my $dir (split(':', $path)) {
        if (-e "$dir/$file" && ! -d "$dir/$file") {
            return("$dir/$file");
        }
    }
    return;
}
__END__
=head1 NAME
latexpand - Flatten LaTeX file by expanding \include and \input, ... and  remove comments
=head1 SYNOPSIS
latexpand [options] FILE...
=head2 Options:
    --verbose        show what's going on
    --keep-comments  don't strip comments (comments are lines
                         starting with %, and anything below
                         \end{document})
    --empty-comments keep empty comments (i.e. % at end of lines) for clarity
    --keep-includes  don't expand \input and \include directives
    --expand-usepackage
                     Expand \usepackage{...} directives if the
                     corresponding .sty file is found in
                     $TEXINPUTS (or the current directory if
                     $TEXINPUTS is not set)
    --expand-bbl FILE
                     Expand the bibliography by inlining FILE
                     (should be a *.bbl file)
    --help           this help message
    --output <file>, -o <file>
                     generate output in <file>
    --explain        generate explanatory comments in output
    --show-graphics  show included graphics
    --graphics_extensions
                     colon-separated list of possible graphics extensions
                     (used by --show-graphics to find the actual graphics files)
    --fatal          Die in case a file can't be found.
    --makeatletter   Insert a \makeatletter in the preamble. In some
                     rare cases it may break your document, but it
                     may help fixing bad interactions between
                     @-commands and inclusion (see BUGS section).

=head1 USES
The most common use of latexpand is to simplify distribution of source
LaTeX files, typically to satisfy the requirement of editors and
archival sites (springer, arXiv.org, ...) who force the authors to
submit sources. One does not necessarily want to submit sources with
comments, and uploading a document made of several files including
each other is a bit painful. By default, latexpand answers both
problems by outputing a single LaTeX file that contain no comment.
=head1 GETTING LATEXPAND
The latest version of latexpand is available here:
  https://gitlab.com/latexpand/latexpand
Versions are uploaded to ctan.org from time to time:
  http://www.ctan.org/pkg/latexpand
=head1 BUGS
Please, report bugs on the issue tracker on the project site:
  https://gitlab.com/latexpand/latexpand/issues
=head2 Known bugs
=head3 Verbatim
latexpand currently ignores \begin{verbatim} ... \end{verbatim}, and
will therefore process any \include, \input, ... directives that
appear within verbatim environments (while it shouldn't).
LaTeX comments inside verbatim environments are also incorrectly
stripped. You can use --keep-comments as a workaround to avoid this.
=head3 Comment environment
It would be nice to remove code between \begin{comment} and
\end{comment} too if \usepackage{comment} is used.
Code like
    foo%
    \begin{comment}
will produce the incorrect
    foo\begin{comment}
A workaround is to use --empty-comments when such tricky usage of the
comments package is done.
=head3 \makeatletter and use with transfig/xfig with \scalebox{}
If \input{} or \include{} appears as argument to a command, and the
file included contains \makeatletter, then after expansion, the
\makeatletter and the @-command appear as argument to the command,
which is forbidden because the argument is parsed (and the @-command
badly tokenized) before being executed.
This happens with
    \scalebox{ \input{file-generated-by-xfig.pdf_t} }
Workaround: add \makeatletter before the scalebox manually in your
code, like
        \makeatletter{}
    \scalebox{ \input{file-generated-by-xfig.pdf_t} }
        \makeatother{}
In the case of xfig generated files, it is necessary only for the
first occurence.
A more brute-force workaround is to use latexpand --makeatletter.
=head1 SEE ALSO
Instructions to include only the relevant .bib items (french):
https://lacl.fr/~caubert/notes/portabilite-du-tex.html#dependances
=head1 VERSION
This is latexpand version v1.4-1-gb32a776.

